Understanding and maintaining tactics graphically OR how we are learning that a diagram can be worth more than 10K LoC

The use of a functional language to implement proof strategies as proof tactics in interactive theorem provers, often provides short, concise and elegant implementations. Whilst being elegant, the use of higher order features and combinator languages often results in a very procedural view of a strategy, which may deviate significantly from the high-level ideas behind it. This can make a tactic hard to understand and hence difficult to to debug and maintain for experts and non-experts alike: one often has to tear apart complex combinations of lower level tactics manually in order to analyse a failure in the overall strategy. In an industrial technology transfer project, we have been working on porting a very large and complex proof tactic into PSGraph, a graphical language for representing proof strategies, supported by the Tinker tool. The goal of this work is to improve understandability and maintainability of tactics. Motivated by some initial successes with this, we here extend PSGraph with additional features for development and debugging. Through the re-implementation and refactoring of several existing tactics, we demonstrates the advantages of PSGraph compared with a typical linear (term-based) tactic language with respect to debugging, readability and maintenance. In order to act as guidance for others, we give a fairly detailed comparison of the user experience with the two approaches. The paper is supported by a web page providing further details about the implementation as well as interactive illustrations of the examples.

==> case_conv.tex <==
% -*- mode: LaTeX; mode: FlySpell; -*-
% !TEX root = jfr.tex

%\comment{TODO: need some text to explain how recursion work in the original tactic}
\subsubsection{The problem of turning conversions into tactics}

PSGraph works with \emph{tactics} and not conversions, and in order to use a conversion in PSGraph a conversion must first be turned into a tactic. Functionality to achieve this
in ProofPower via 
\begin{GFT}{SML}
\+ val conv\_tac : CONV -> TACTIC\\
\end{GFT}
Using this function we can for example turn our \emph{rec\_conv} conversion into a tactic:
\begin{GFT}{SML}
\+ val conv\_rec\_tac : TACTIC = conv\_tac rec\_conv\\
\end{GFT}
As we have seen, combinators has a set of \emph{conversion combinators}, comparable to tacticals for tactics, in order to combine conversions. As in the previous case studies, 
we need to find suitable representations for this in PSGraph. However, this is not straightforward as we are not working with conversions and not tactics. For some examples
we can explore certain algebraic laws, and ``lift" conversions combinators to tactics, as exemplified for sequential composition:  
$$
conv\_tac (c_1~\textit{THEN\_C}~c_2) = (conv\_tac~c_1)~\textit{THEN}~(conv\_tac~c_2)
$$
We can then use the same approach as before and turn $conv\_tac~c_1$ and $conv\_tac~c_2$ into atomic tactics with a wire between them. However, conversions are typically applied
to sub-terms of the goal, and certain combinators are used to change ``the focus'' of the conversion to a sub-term. For example, given a 
term $\PrKM{}f x\PrKO{}$, \emph{RAND\_C} will change the focus to the sub-term $\PrKM{}x\PrKO{}$.
To illustrate, $\emph{RAND\_C}~(c_1~\textit{THEN\_C}~c_2)$ will first change the focus of the term, and then apply $c_1$ followed by $c_2$ to this sub-term.

We cannot naively break up the \textit{THEN\_C} combinator into the \textit{THEN} tactical, as $c_2$ should work on the sub-term as a result of the use of \emph{RAND\_C}.
For this case, we could again develop suitable algebraic laws and ``push'' \emph{RAND\_C} inwards, i.e. $(\emph{RAND\_C}~c_1)~\textit{THEN\_C}~(\emph{RAND\_C}~c_2)$,
and then use the same approach to turn this into a tactic. However, a deeper problem for $rec\_conv$ is the recursion: in most cases the term focus is changed followed by
a recursive application of the same conversion. When the recursion terminates, then some further work has to be done (at the ``focus'' before the call). 
In PSGraph we represent repetition, such as recursion, using a feedback loop. However, in this case we need to keep track of the current focus of the term for each iteration,
as well as knowing where the focus was beforehand on exist.


\subsubsection{Encoding recursion with ``term focusing''in PSGraph}

\begin{figure}
\begin{center}
\includegraphics[width=0.7\textwidth]{psgraph_images/conv/rec_conv_full} 
\end{center}
\vspace{-15pt}
\caption{Encoding recursion with ``term focusing'' in PSGraph}
\label{fig:conv:rec}
\end{figure}


%Conversion is an important concept to facilitate tactic development. A conversion is a function turning a given term to a theorem, i.e.
% \begin{GFT}{SML}
% \+	type CONV = TERM -> THM\\ 
% \end{GFT}



Our solution to implement the \emph{rec\_conv} conversion, is to augment the PSGraph with a variable $?rec$ acting like a stack that keeps track of
each change of focus to a term when entering a recursive step. This variable has type\footnote{We have updated the allowed types in an environment for simplicity -- we could just
as well used a list of names, and developed a parser to turn this into a conversion.}
\begin{GFT}{}
\+  ?rec : (CONV -> CONV) list\\
\end{GFT}
The idea is as follows. For each application of a conversion, we first sequentially compose all element of $?rec$ and apply this to focus the correct place in a term followed by the
application of a term. We specialise \emph{conv\_tac} with a tactic that takes these two arguments:
\begin{GFT}{ML}
\+ lift\_conv: (CONV -> CONV) list -> CONV -> tactic\\
\end{GFT}
If this conversion is followed by a recursive application, then the ``term focus combinators'' are pushed to the $?rec$ stack. This is achieved by an environment tactic 
\emph{ENV\_push(conv,var)}, which takes one of these conversion combinators and a variable as argument. 

Afterwards, the operations after the recursion is applied in a loop. It will again uses $?rec$, and apply the operations followed by popping an element of it until $?rec$ is empty.
The environment tactic \emph{ENV\_pop(var)} is used to pop one element of the stack which $var$ refers to. As can be seen in the definition of \emph{rec\_conv}, the post operations are
always an application of \emph{simp\_conv}, so we only need to keep track of the focus and not which conversion to apply at each point.

The encoding of this strategy is shown in Fig. \ref{fig:conv:rec}. It takes an input a goal with an environment containing a variable $?cc$ with the current focus, and initialises $?rec$
to this value. The $i\_conv$ and $k\_conv$ conversions are applied without any recursion, as described above. For the other cases, the \emph{recursion} graph tactic is added. For each case
conversion $c$, i.e. each element of the list of \emph{rec\_conv} we develop an atomic goal type, called \emph{is\_c\_conv}. For the graph tactic, \emph{is\_rec\_conv} is just the disjunction
of the four recursive cases:
$$
\begin{array}{lcl}
is\_rec\_conv(X) & \leftarrow &  is\_unary\_conv(X).\\
is\_rec\_conv(X) & \leftarrow &  is\_param\_conv(X).\\
is\_rec\_conv(X) & \leftarrow &  is\_binary\_conv(X).\\
is\_rec\_conv(X) & \leftarrow &  is\_pair\_conv(X).
\end{array}
$$
In each of the case, the conversion is applied and then the focus of the term is changed. For example \emph{pair\_conv} is followed by two application of \emph{RAND\_C} and then a recursive call
again to \emph{rec\_conv}. Thus, for this case, $\textit{RAND\_C} \circ \textit{RAND\_C}$ is added to $?rec$. 

The recursion stops when there are more conversions that applies, i.e. none of the goal types succeeds. This is the negation of the case where any of the conversion goal types are satisfied, i.e.:
$$
\begin{array}{lcl}
more\_conv(X) & \leftarrow &  is\_i\_conv(X).\\
more\_conv(X) & \leftarrow &  is\_k\_conv(X).\\
more\_conv(X) & \leftarrow &  is\_rec\_conv(X).
\end{array}
$$
On exit, the last change of focus is removed (as it failed for this application), and we enter the \emph{post\_recursion} graph tactic, unless the case where $?rec$ is still the same as $?cc$ (i.e. none of the calls succeeded).
In this graph tactic the \emph{simp\_conv} will be applied for the same sub-terms as in the recursive case (due to the feedback loop around the tactic). When $?rec$ is the same as $?cc$, this loop terminated. This concludes the proof 
strategy.


% We are essentially providing an argument.


% One possible solution is to introduce two loops for each recursion, one loop locates before the point where recursion happens and the other one locates after the point, i.e. the graph nodes \emph{recursion} and \emph{post\_recursion}in Figure \ref{fig:conv:rec}. In each iteration, conversion is applied combined with a conversion combinator which is accumulated through recursion. Therefore, we introduce an env var to accumulate the effect of the conversion combinators, i.e.



% In each iteration of the recursion, one conversion combinator is pushed to $?rec$. This is supported by the env tactic, i.e. 
% \begin{GFT}{}
% \+  ENV\_push: (CONV -> CONV) -> Variable\\
% \end{GFT}
% \noindent
% where $A\_Var$ is a env var which keep tracks of the current focus of the sub-term by storing the combinators in a list, i.e. the the type of the instance of the env var is  $(CONV -> CONV) list$. Therefore, when a goal node is evaluated with a $ENV\_push$ env tactic node, e.g., $ENV\_push(cc, v)$, Tinker will get lookup variable $i$ in the environment of the goal node to get the combinator list, then to push the new combinator $v$ in the list and to update variable $i$ with the new list.


% Similarly, in each iteration of post recursion, the head element of $?rec$ is popped, which is supported by
% \begin{GFT}{}
% \+  ENV\_pop: A\_Var -> env -> env list\\
% \end{GFT}
%  In this way, we can synchronise the number of iteration for two loops during evaluation.

% To order to apply conventions with an argument of $(CONV -> CONV) list$ ,  we also define a new conversion lift function, i.e. 

% \begin{GFT}{}
% \+ lift\_conv: (CONV -> CONV) list -> CONV -> tactic\\
% \end{GFT}
% which first folds the all conversion combinators in $?rec$ with the conversion to produce a new conversion, then to act as $conv\_tac$.


			


==> case_fef.tex <==
\comment{TODO: some background of fef project and description of tac1 ... tac4 (Rob) }

The targeted tactics in \texttt{ML}: 
\begin{GFT}{SML}
\footnotesize
\+val tac1 = REPEAT strip\_tac THEN\\
\+	LEMMA\_T \PrKM{}Snd x \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+	(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])\\
\+	THEN1 PC\_T1 "sets\_ext" asm\_prove\_tac(map get\_spec[\PrKM{}Elems\PrKO{}, \PrKM{}Map\PrKO{}]);\\
\+\\
\+val tac2 = REPEAT strip\_tac THEN\\
\+	cases\_tac\PrKM{}Snd (te tl\PrIJ{0} rl\PrIJ{0} r\PrIJ{0}) = Snd (te tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1})\PrKO{}\\
\+	THEN\_LIST [\\
\+	asm\_ante\_tac \PrKM{}\PrLD{} Snd (te tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1}) = Snd (Fst x tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1})\PrKO{}\\
\+	THEN POP\_ASM\_T (asm\_rewrite\_thm\_tac o eq\_sym\_rule)\\
\+	THEN REPEAT strip\_tac THEN\\
\+	LEMMA\_T \PrKM{}Fst x \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+		(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])\\
\+	THEN1 PC\_T1 "sets\_ext" asm\_prove\_tac(map get\_spec[\PrKM{}Elems\PrKO{}, \PrKM{}Map\PrKO{}]),\\
\+	DROP\_ASM\_T \PrKM{}te \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+	(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])];\\
\+\\
\+val tac3 = REPEAT strip\_tac THEN\\
\+	cases\_tac\PrKM{}Snd (te tl\PrIJ{0} rl\PrIJ{0} r\PrIJ{0}) = Snd (te tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1})\PrKO{}\\
\+	THEN\_LIST [\\
\+	asm\_ante\_tac \PrKM{}\PrLD{} Snd (te tl\PrIJ{0} rl\PrIJ{0} r\PrIJ{0}) = Snd (Fst x tl\PrIJ{0} rl\PrIJ{0} r\PrIJ{0})\PrKO{}\\
\+	THEN asm\_rewrite\_tac[]\\
\+	THEN STRIP\_T (asm\_tac o conv\_rule(RAND\_C eq\_sym\_conv)) THEN\\
\+	LEMMA\_T \PrKM{}Fst x \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+		(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])\\
\+	THEN1 PC\_T1 "sets\_ext" asm\_prove\_tac(map get\_spec[\PrKM{}Elems\PrKO{}, \PrKM{}Map\PrKO{}]),\\
\+	DROP\_ASM\_T \PrKM{}te \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+	(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])];\\
\+\\
\+val tac4 = REPEAT strip\_tac THEN\\
\+	DROP\_ASM\_T \PrKM{}CaseVal c te cel ee \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+	(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th]);\\
\end{GFT}
\comment{assume that these definitions are covered in the above explanation}

\subsubsection{Encoding similarities as patterns}
We observe that the definitions of the four tactics in \emph{fef} share similarities. Thus, one efficient approach to develop the fef tactics in PSGraph is to generalise the similarities as patterns and encode each pattern into a PSGraphs. The fef tactics can then be incrementally developped by reusing these PSGraphs. To ease presentation, we name the three patterns as \emph{LEMMA\_THEN1}, \emph{CASE\_THENLIST} and \emph{DROP\_ASM}. The \texttt{ML} code definition of these patterns are:

\begin{tabular}{lcl}
	LEMMA\_THEN1 &:& \emph{(LEMMA\_T ?goal ?thm\_tac) THEN1 ?tac} \\
	CASE\_THENLIST &:& \emph{case\_tac ?case THEN\_LIST[?tac1, ?tac2]} \\ 
	DROP\_ASM &:& \emph{DROP\_ASM\_T ?assum thm\_tac}\\
\end{tabular}

\noindent where generalised parts start with question marks ($?$). We will discuss each pattern in order as follows. 

Pattern LEMMA\_THEN1 shows common proof steps that adding a new subgoal with term \emph{?g} and then applying tactic \emph{?tac} to this new subgoal, followed by applying tactic \emph{?thm\_tac (?goal} $\vdash$ \emph{?goal)} to the original goal. This pattern is used in \emph{tac1} which are:
\begin{GFT}{SML}
\+ (fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])\\
\end{GFT}
\noindent and 
\begin{GFT}{SML}
\+ PC\_T1 "sets\_ext" asm\_prove\_tac(map get\_spec[\PrKM{}Elems\PrKO{}, \PrKM{}Map\PrKO{}]);\\
\end{GFT}
\noindent respectively.

To parametrise $?goal$ for this pattern in PSGraph, we introduce a \emph{pvar} $?g$ and an \emph{env tac} node to assign an appropriate term to $?g$, also for the tactic nodes which need to be updates when the pattern is used to develop fef tactics, their names start with \emph{config}. Fig.~\ref{fig:fef:lemmat} shows the PSGraph version of this pattern as a graph tactic where the top level is on the left and the sub-graphs of the graph node is on the right. 

Firstly, the env tac node 
\emph{?g:= @\{term ``XXX''\}} binds a pvar $?g$ with an appropriate term in the goal node which flows through the env tac node. Then $lemma\_tac (?g)$ adds a new subgoal using the term in pvar $?g$. The goal types on the output edge of $lemma\_tac (?g)$, i.e. $is\_goal(?g)$ and $is\_not\_goal(?g)$, guide the subgoal to the right upcoming node by checking whether the goal term is  the same as the one in pvar $?g$.  The new subgoal which is the same as $?g$, is then sent to output edge with the subsequent node \emph{config\_tac};  the original subgoal, is then sent to the other output edge. From the env tac node \emph{?gThm := @\{thm ``asm\_rule ?g''\}}, this subgoal gets a new pvar $?gThm$ in its env with the thm of \emph{asm\_rule ?g}, which is semantically the same as $?g \vdash ?g$. After that, \emph{dummy\_thm\_tac (?gThm)} is then applied to the subgoal. Node that, \emph{XXX} and the atomic nodes which starts with \emph{dummy} are expected to be updated when this PSGraph of \emph{LEMMA\_THEN1} is used in developing the fef tactics.

\begin{figure}
\begin{center}
\includegraphics[width=0.23\textwidth]{psgraph_images/fef/lemmatl} 
$\quad \quad \quad \quad$
\includegraphics[width=0.4\textwidth]{psgraph_images/fef/lemmatr} 
\end{center}
\caption{PSGraph encoding of \emph{LEMMA\_THEN1}}
\label{fig:fef:lemmat}
\end{figure}
%\comment{explain why REPEAT stri\_tac become a atomic tac}

Similar to \emph{LEMMA\_THEN1}, we can also develop \emph{CASE\_THENLIST} and \emph{DROP\_ASM} as graph node. For \emph{CASE\_THENLIST}, it is a proof pattern that applying a case split on term \emph{?case}, and then apply \emph{?tac1} to the subgoal with the hypothesis of \emph{?case}, and \emph{?tac2} to the other. The PSGraph version of \emph{CASE\_THENLIST} is shown is Fig~\ref{fig:fef:case}.

For \emph{DROP\_ASM}, it first applies a tactic, \emph{config\_tac}, using the hypothesis \emph{?hyp} and then remove the hypothesis. Figure \ref{fig:fef:drop} shows the PSGraph version.

\comment{Goal type for current version (we should actually use not()) does not handle all cases, as proofpower may do simplify/split sub-goals. We should make a point that this will not happen here and think about the future.}

\begin{figure}
\begin{center}
\includegraphics[width=0.25\textwidth]{psgraph_images/fef/casel} 
$\quad \quad \quad \quad$
\includegraphics[width=0.33\textwidth]{psgraph_images/fef/caser} 
\end{center}
\caption{PSGraph encoding of \emph{CASE\_THENLIST}}
\label{fig:fef:case}
\end{figure}


\begin{figure}
\begin{center}
\includegraphics[width=0.25\textwidth]{psgraph_images/fef/dropl} 
$\quad \quad \quad \quad$
\includegraphics[width=0.3\textwidth]{psgraph_images/fef/dropr} 
\end{center}
\caption{PSGraph encoding of \emph{DROP\_ASM}}
\label{fig:fef:drop}
\end{figure}

\subsubsection{Developing tactics with a top-down approach}
We can save the PSGraph of these patterns into the library of Tinker \cite{Lin2016}, so that patterns can be imported to develop the fef tactics in a modular way. For simpler tactics, such as tac1 and tac4, only one pattern is needed. Take \emph{tac1} for example, Figure.\ref{fig:fef:tac1} shows the PSGraph version, it can be developed using $LEMMA\_THEN1$ by assigning the initial value
\begin{GFT}{SML}
\+\PrKM{}Snd x \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\end{GFT}
 to \emph{?g}, and updating \emph{config\_tac} to \emph{PC\_T1\_asm\_prove\_tac} which is
\begin{GFT}{SML}
\+ PC\_T1 "sets\_ext" asm\_prove\_tac(map get\_spec[\PrKM{}Elems\PrKO{}, \PrKM{}Map\PrKO{}]);\\
\end{GFT}
\noindent and updating \emph{dummy\_thm\_tac} to \emph{asm\_fc\_thm\_tac(?gThm)} which is 
\begin{GFT}{SML}
\+ all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}]) ?gThm]\\
\end{GFT}

\begin{figure}
\begin{center}
\includegraphics[width=0.3\textwidth]{psgraph_images/fef/tac1l} 
$\quad \quad \quad \quad$
\includegraphics[width=0.4\textwidth]{psgraph_images/fef/tac1r} 
\end{center}
\caption{PSGraph \emph{tac1}: top level (left) and the sub-graphs of node \emph{LEMMA\_THEN1(?g)}(right)}
\label{fig:fef:tac1}
\end{figure}

For more complicated tactics, such as \emph{tac2} and \emph{tac3}, a top-down approach can be adopted. We will demonstrate this approach with \emph{tac2}. Let us first recall the ML definition with some boxes to highlight patterns:

\begin{center}
\includegraphics[width=\textwidth]{psgraph_images/fef/tac_anno} 
\end{center}

where the green box highlight the \emph{CASE\_THENLIST} pattern, the red boxes highlight two tactics for the positive and negative cases in \emph{CASE\_THENLIST}. For the tactic in the first red box, part of it uses the \emph{LEMMA\_THEN1} pattern, as highlighted in the blue box; the tactic in the second red box follows the \emph{DROP\_ASM} pattern.

\begin{figure}
\begin{center}
\includegraphics[width=0.25\textwidth]{psgraph_images/fef/tac2_l0} 
$\quad$
\includegraphics[width=0.4\textwidth]{psgraph_images/fef/tac2_l1} 
$\quad$
\includegraphics[width=0.25\textwidth]{psgraph_images/fef/tac2_neg} 
\end{center}
\caption{The top, second level and subgraphs of DROP\_ASM  of tac2 in PSGraph}
\label{fig:fef:tac2 1st and 2nd}
\end{figure}


To develop the PSGraph version of tac2, firstly the \emph{CASE\_THENLIST} pattern is imported at the top level with initialisation of \emph{?case} to
\begin{GFT}{SML}
\footnotesize
\+\PrKM{}Snd (te tl\PrIJ{0} rl\PrIJ{0} r\PrIJ{0}) = Snd (te tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1})\PrKO{}\\
\end{GFT}

For the tactics nodes $config\_pos$ and $config\_neg$, i.e. the tactics to handle the positive case and negative case, two graph tactic nodes are inserted for further decomposition, as shown in Figure \ref{fig:fef:tac2 1st and 2nd}.

For the tactic of the negative case which is highlighted by the second red box, it follows \emph{DROP\_ASM}. The corresponding PSGraph is inserted with initialisation of \emph{?hyp} to
\begin{GFT}{SML}
\+\PrKM{}te \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\end{GFT}
\noindent and updating \emph{config\_tac(?hyp)} to \emph{asm\_fc\_thm\_tac(?hyp)} which is
\begin{GFT}{SML}
\+	all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}]) ?hyp])\\	
\end{GFT}
\noindent
The sub-graph development for the proof of negative case is completed, which is shown in  \ref{fig:fef:tac2 1st and 2nd}.

% \begin{figure}
% \begin{center}
% \includegraphics[width=0.3\textwidth]{psgraph_images/fef/tac2_neg} 
% \end{center}
% \caption{Sub-graph of $DROP\_ASM$}
% \label{fig:fef:tac22neg}
% \end{figure}

To decomposite the tactic of the positive case, which is highlighted by the first red box, and develop the sub-graph $POS\_CASE$, 
% \+val tac2 = REPEAT strip\_tac THEN\\
% \+	cases\_tac\PrKM{}Snd (te tl\PrIJ{0} rl\PrIJ{0} r\PrIJ{0}) = Snd (te tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1})\PrKO{}\\
% \+	THEN\_LIST [\\
% \+	asm\_ante\_tac \PrKM{}\PrLD{} Snd (te tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1}) = Snd (Fst x tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1})\PrKO{}\\
% \+	THEN POP\_ASM\_T (asm\_rewrite\_thm\_tac o eq\_sym\_rule)\\
% \+	THEN REPEAT strip\_tac THEN\\
% \+	LEMMA\_T \PrKM{}Fst x \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
% \+		(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])\\
% \+	THEN1 PC\_T1 "sets\_ext" asm\_prove\_tac(map get\_spec[\PrKM{}Elems\PrKO{}, \PrKM{}Map\PrKO{}]),\\
% \+	DROP\_ASM\_T \PrKM{}te \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
% \+	(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])];\\
% \+\\
we first implement 
\begin{GFT}{SML}
\+asm\_ante\_tac \PrKM{}\PrLD{} Snd (te tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1}) = Snd (Fst x tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1})\PrKO{}\\
\end{GFT}
as an tactic node 
$asm_ante_tac(?z)$, where $?z$ is a pvar with the value of
\begin{GFT}{SML}
\+ \PrKM{}\PrLD{} Snd (te tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1}) = Snd (Fst x tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1})\PrKO{}\\
\end{GFT}

the sub-tactic, i.e. \emph{POP\_ASM\_T (asm\_rewrite\_thm\_tac o eq\_sym\_rule)}, as an sequential application of 
$rewrite_sym_thm_tac(?case)$, $rewrite_sym_thm_tac(?case)$ and $default_asm_rewrite_tac$. The remaining part are the same as \emph{tac1}, i.e. it can be developed by using the \emph{LEMMA\_THEN1} pattern. This version of $POS\_CASE$
is shown in Fig~\ref{fig:fef:tac22pos} (left). By grouping for its original sub-tactics, a hierarchical version can be developed, as shown in Fig~\ref{fig:fef:tac22pos} (right). 

\begin{figure}
\begin{center}
\includegraphics[width=0.3\textwidth]{psgraph_images/fef/tac2_pos_v1} 
$\quad \quad$
\includegraphics[width=0.3\textwidth]{psgraph_images/fef/tac2_pos_v2} 
\end{center}
\caption{A flat version $POS\_CASE$ (LEFT) and a hierarchical version$POS\_CASE$ (right)}
\label{fig:fef:tac22pos}
\end{figure}

\subsubsection{Refactoring when requirement changes (remove this ?)}
\comment{need some details of the experiment from Rob}



==> case_fef_raw.tex <==
\begin{GFT}{SML}
\+val tac1 = REPEAT strip\_tac THEN\\
\+	LEMMA\_T \PrKM{}Snd x \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+	(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])\\
\+	THEN1 PC\_T1 "sets\_ext" asm\_prove\_tac(map get\_spec[\PrKM{}Elems\PrKO{}, \PrKM{}Map\PrKO{}]);\\
\+\\
\+val tac2 = REPEAT strip\_tac THEN\\
\+	cases\_tac\PrKM{}Snd (te tl\PrIJ{0} rl\PrIJ{0} r\PrIJ{0}) = Snd (te tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1})\PrKO{}\\
\+	THEN\_LIST [\\
\+	asm\_ante\_tac \PrKM{}\PrLD{} Snd (te tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1}) = Snd (Fst x tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1})\PrKO{}\\
\+	THEN POP\_ASM\_T (asm\_rewrite\_thm\_tac o eq\_sym\_rule)\\
\+	THEN REPEAT strip\_tac THEN\\
\+	LEMMA\_T \PrKM{}Fst x \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+		(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])\\
\+	THEN1 PC\_T1 "sets\_ext" asm\_prove\_tac(map get\_spec[\PrKM{}Elems\PrKO{}, \PrKM{}Map\PrKO{}])\\
\+	,\\
\+	DROP\_ASM\_T \PrKM{}te \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+	(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])];\\
\+val tac3 = REPEAT strip\_tac THEN\\
\+	cases\_tac\PrKM{}Snd (te tl\PrIJ{0} rl\PrIJ{0} r\PrIJ{0}) = Snd (te tl\PrIJ{1} rl\PrIJ{1} r\PrIJ{1})\PrKO{}\\
\+	THEN\_LIST [\\
\+	asm\_ante\_tac \PrKM{}\PrLD{} Snd (te tl\PrIJ{0} rl\PrIJ{0} r\PrIJ{0}) = Snd (Fst x tl\PrIJ{0} rl\PrIJ{0} r\PrIJ{0})\PrKO{}\\
\+	THEN asm\_rewrite\_tac[]\\
\+	THEN STRIP\_T (asm\_tac o conv\_rule(RAND\_C eq\_sym\_conv)) THEN\\
\+	LEMMA\_T \PrKM{}Fst x \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+		(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])\\
\+	THEN1 PC\_T1 "sets\_ext" asm\_prove\_tac(map get\_spec[\PrKM{}Elems\PrKO{}, \PrKM{}Map\PrKO{}])\\
\+	,\\
\+	DROP\_ASM\_T \PrKM{}te \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+	(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th])];\\
\+val tac4 = REPEAT strip\_tac THEN\\
\+	DROP\_ASM\_T \PrKM{}CaseVal c te cel ee \PrIN{} OK\_VC\PrIJ{d} c\PrKO{}\\
\+	(fn th => all\_fc\_tac[rewrite\_rule(map get\_spec[\PrKM{}OK\_VC\PrIJ{d}\PrKO{}])th]);\\
\end{GFT}

